FrontierCS 2: A Benchmark for Computer Science R&D

Can LLM agents make contributions to frontier computer science R&D? We introduce FrontierCS 2, a benchmark of 48 open-ended tasks. We take a paper and the code its authors released and delete the paper's contribution. The deleted code becomes the human reference that sets the bar. Earlier open-ended benchmarks give each agent a problem statement and grade one program after the run. FrontierCS 2 places the agent inside a research environment. The agent inherits a working repository and may submit a patch at any point. For each patch, a judge returns a development-suite score but keeps the evaluator, the held-out final suite and the reference private, and grades the final submission on that suite against the reference. The tasks span 13 domains, from machine-learning systems and high-performance computing to databases, security and robotics. Beyond these 48 tasks, FrontierCS 2 keeps a private set of more than 100 tasks, to be announced in the future. We evaluate 12 agents. The best one is Claude Opus 5.5, passing 58% of its runs. No run passes on 16 tasks. A higher score is not the same as a pass: most runs that beat the reference on the combined final score still fall short on some metric or workload. On a shared capability scale for agents and tasks, the median task is roughly as difficult as what the strongest agent can handle.

==> packages.tex <==
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{mathtools}                %
\RequirePackage{bm}                       %
\RequirePackage{mathpazo}

\RequirePackage{microtype}
\RequirePackage{anyfontsize}
\RequirePackage{titlesec}
\RequirePackage{tocloft}
\RequirePackage[defaultsans]{lato}        %

\RequirePackage{xcolor}
\RequirePackage{colortbl}
\definecolor{gblue}{HTML}{1A73E8}     %
\definecolor{gred}{HTML}{D93025}      %
\definecolor{gyellow}{HTML}{E37400}   %
\definecolor{ggreen}{HTML}{1E8E3E}    %
\definecolor{gpurple}{HTML}{9334E6}   %
\definecolor{ggrey}{HTML}{5F6368}     %
\colorlet{linkcol}{gblue}

\RequirePackage{graphicx}
\RequirePackage{wrapfig}
\RequirePackage{adjustbox}
\RequirePackage{tikz}                     %

\RequirePackage[labelsep=colon]{caption}
\RequirePackage{subcaption}               %

\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{makecell}

\RequirePackage{geometry}
\RequirePackage{fancyhdr}
\RequirePackage{authblk}
\RequirePackage{enumitem}
\RequirePackage{tcolorbox}

\RequirePackage{verbatim}
\RequirePackage{pifont}

\RequirePackage[ruled,vlined,linesnumbered]{algorithm2e}

\RequirePackage[numbers,sort&compress]{natbib}

\RequirePackage[colorlinks=true,allcolors=linkcol]{hyperref}
\RequirePackage[capitalize,noabbrev]{cleveref} %

